Calibration of Time-Series Forecasting: Detecting and Adapting Context-Driven Distribution Shift

Recent years have witnessed the success of introducing deep learning models to time series forecasting. From a data generation perspective, we illustrate that existing models are susceptible to distribution shifts driven by temporal contexts, whether observed or unobserved. Such context-driven distribution shift (CDS) introduces biases in predictions within specific contexts and poses challenges for conventional training paradigms. In this paper, we introduce a universal calibration methodology for the detection and adaptation of CDS with a trained model. To this end, we propose a novel CDS detector, termed the "residual-based CDS detector" or "Reconditionor", which quantifies the model's vulnerability to CDS by evaluating the mutual information between prediction residuals and their corresponding contexts. A high Reconditionor score indicates a severe susceptibility, thereby necessitating model adaptation. In this circumstance, we put forth a straightforward yet potent adapter framework for model calibration, termed the "sample-level contextualized adapter" or "SOLID". This framework involves the curation of a contextually similar dataset to the provided test sample and the subsequent fine-tuning of the model's prediction layer with a limited number of steps. Our theoretical analysis demonstrates that this adaptation strategy can achieve an optimal bias-variance trade-off. Notably, our proposed Reconditionor and SOLID are model-agnostic and readily adaptable to a wide range of models. Extensive experiments show that SOLID consistently enhances the performance of current forecasting models on real-world datasets, especially on cases with substantial CDS detected by the proposed Reconditionor, thus validating the effectiveness of the calibration approach.

==> main_table.tex <==
\newcommand{\rotate}[1]{\begin{tabular}{@{}c@{}}\multirow{6}{*}{{\rotatebox[origin=c]{90}{#1}}}\end{tabular}}

\begin{table*}[htbp]
  \centering
  \caption{Performance of our proposed methods. "$\bm \uparrow$": average improvements achieved by \method{\textit{SOLID}} compared to the original forecasting results. "$\bm \delta$": metrics given by \method{\textit{Reconditioner}} in two observed contexts: periodic phases ($\bm{\delta_P}$) and temporal segments ($\bm{\delta_T}$), presented in the form of $\bm{\log_{10} \delta_P\ \&\ \log_{10} \delta_T}$. \textcolor[rgb]{1,0,0}{RED} highlights a \textit{strong} CDS in periodic phases (\ie, $\bm{\log_{10} \delta_P\geq -3.2}$), while \textcolor[rgb]{ 0,  .439,  .753}{BLUE} highlights a \textit{weak} CDS in periodic phases (\ie, $\bm{\log_{10} \delta_P< -3.2}$).}
    \resizebox{\linewidth}{!}{  % 此处！表示根据根据宽高比进行自适应缩放，并且一定要加载tabular两端，而不是table两端。
    \begin{tabular}{c|c|cccc|cccc|cccc|cccc|cccc}
    \toprule
    \multicolumn{2}{c|}{\textbf{Method}}       & \multicolumn{2}{c}{\textbf{Crossformer}} & \multicolumn{2}{c|}{\textbf{+\method{SOLID}}} & \multicolumn{2}{c}{\textbf{ETSformer}} & \multicolumn{2}{c|}{\textbf{+\method{SOLID}}} & \multicolumn{2}{c}{\textbf{FEDformer}} & \multicolumn{2}{c|}{\textbf{+\method{SOLID}}} & \multicolumn{2}{c}{\textbf{Autoformer}} & \multicolumn{2}{c|}{\textbf{+\method{SOLID}}} & \multicolumn{2}{c}{\textbf{Informer}} & \multicolumn{2}{c}{\textbf{+\method{SOLID}}} \\
    \midrule
    \multicolumn{2}{c|}{\textbf{Metric}} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} \\
    \midrule
    \midrule
        \rotate{\textbf{Illness}} & \textbf{24 } & 3.329  & 1.275  & \textbf{2.353 } & \textbf{0.986 } & 2.397  & 0.993  & \textbf{2.262 } & \textbf{0.955 } & 3.241  & 1.252  & \textbf{2.707 } & \textbf{1.123 } & 3.314  & 1.245  & \textbf{2.737 } & \textbf{1.118 } & 5.096  & 1.533  & \textbf{2.874 } & \textbf{1.150 } \\
          & \textbf{36 } & 3.392  & 1.185  & \textbf{2.527 } & \textbf{1.042 } & 2.504  & 0.970  & \textbf{2.301 } & \textbf{0.934 } & 2.576  & 1.048  & \textbf{2.365 } & \textbf{0.990 } & 2.733  & 1.078  & \textbf{2.540 } & \textbf{1.015 } & 5.078  & 1.535  & \textbf{3.299 } & \textbf{1.243 } \\
          & \textbf{48 } & 3.481  & 1.228  & \textbf{2.499 } & \textbf{1.063 } & 2.488  & 0.999  & \textbf{2.320 } & \textbf{0.961 } & 2.546  & 1.058  & \textbf{2.435 } & \textbf{1.023 } & 2.651  & 1.075  & \textbf{2.455 } & \textbf{1.042 } & 5.144  & 1.567  & \textbf{2.879 } & \textbf{1.169 } \\
          & \textbf{60 } & 3.571  & 1.234  & \textbf{3.103 } & \textbf{1.199 } & 2.494  & 1.011  & \textbf{2.358 } & \textbf{1.002 } & 2.784  & 1.136  & \textbf{2.677 } & \textbf{1.118 } & 2.848  & 1.126  & \textbf{2.689 } & \textbf{1.082 } & 5.243  & 1.582  & \textbf{3.773 } & \textbf{1.394 } \\
\cmidrule{2-22}          & \textbf{$\uparrow$} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{23.89\%} & \textbf{12.84\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{6.50\%} & \textbf{3.03\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{8.64\%} & \textbf{5.34\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{9.75\%} & \textbf{5.90\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{37.62\%} & \textbf{20.29\%} \\
          & $\delta$ & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-1.038 \& -0.917}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-1.544 \& -1.001}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-1.099 \& -0.917}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-1.166 \& -1.016}}} & \multicolumn{4}{c}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-1.096 \& -1.148}}} \\
    \midrule
    \midrule
    \rotate{\textbf{Electricity}} & \textbf{96 } & 0.184  & 0.297  & \textbf{0.182 } & \textbf{0.295 } & 0.187  & 0.304  & \textbf{0.171 } & \textbf{0.285 } & 0.188  & 0.304  & \textbf{0.172 } & \textbf{0.284 } & 0.207  & 0.324  & \textbf{0.189 } & \textbf{0.304 } & 0.321  & 0.407  & \textbf{0.245 } & \textbf{0.355 } \\
          & \textbf{192 } & 0.219  & 0.317  & \textbf{0.216 } & \textbf{0.314 } & 0.198  & 0.313  & \textbf{0.184 } & \textbf{0.298 } & 0.197  & 0.311  & \textbf{0.180 } & \textbf{0.290 } & 0.221  & 0.334  & \textbf{0.205 } & \textbf{0.316 } & 0.351  & 0.434  & \textbf{0.256 } & \textbf{0.363 } \\
          & \textbf{336 } & 0.238  & 0.348  & \textbf{0.235 } & \textbf{0.343 } & 0.210  & 0.326  & \textbf{0.197 } & \textbf{0.312 } & 0.213  & 0.328  & \textbf{0.195 } & \textbf{0.307 } & 0.244  & 0.350  & \textbf{0.232 } & \textbf{0.337 } & 0.349  & 0.432  & \textbf{0.279 } & \textbf{0.381 } \\
          & \textbf{720 } & 0.274  & 0.373  & \textbf{0.269 } & \textbf{0.368 } & 0.249  & 0.356  & \textbf{0.234 } & \textbf{0.341 } & 0.243  & 0.352  & \textbf{0.228 } & \textbf{0.336 } & 0.285  & 0.381  & \textbf{0.273 } & \textbf{0.370 } & 0.385  & 0.493  & \textbf{0.327 } & \textbf{0.416 } \\
\cmidrule{2-22}          & \textbf{$\uparrow$} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{1.42\%} & \textbf{1.11\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{6.89\%} & \textbf{4.75\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{7.88\%} & \textbf{5.95\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{6.16\%} & \textbf{4.44\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{21.28\%} & \textbf{14.21\%} \\
          & $\delta$ & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-2.333 \& -2.42}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-2.559 \& -2.724}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-2.967 \& -2.545}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-2.408 \& -2.134}}} & \multicolumn{4}{c}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-2.975 \& -2.593}}} \\
    \midrule
    \midrule
    \rotate{\textbf{Traffic}} & \textbf{96 } & 0.521  & 0.297  & \textbf{0.473 } & \textbf{0.277 } & 0.599  & 0.386  & \textbf{0.487 } & \textbf{0.354 } & 0.574  & 0.356  & \textbf{0.513 } & \textbf{0.344 } & 0.621  & 0.391  & \textbf{0.565 } & \textbf{0.376 } & 0.731  & 0.406  & \textbf{0.628 } & \textbf{0.393 } \\
          & \textbf{192 } & 0.523  & 0.298  & \textbf{0.475 } & \textbf{0.280 } & 0.611  & 0.391  & \textbf{0.492 } & \textbf{0.354 } & 0.612  & 0.379  & \textbf{0.549 } & \textbf{0.361 } & 0.666  & 0.415  & \textbf{0.599 } & \textbf{0.379 } & 0.739  & 0.414  & \textbf{0.653 } & \textbf{0.413 } \\
          & \textbf{336 } & 0.530  & 0.300  & \textbf{0.481 } & \textbf{0.286 } & 0.619  & 0.393  & \textbf{0.501 } & \textbf{0.359 } & 0.618  & 0.379  & \textbf{0.557 } & \textbf{0.363 } & 0.649  & 0.405  & \textbf{0.595 } & \textbf{0.390 } & 0.850  & 0.476  & \textbf{0.758 } & \textbf{0.466 } \\
          & \textbf{720 } & 0.573  & 0.313  & \textbf{0.498 } & \textbf{0.298 } & 0.629  & 0.391  & \textbf{0.529 } & \textbf{0.374 } & 0.629  & 0.382  & \textbf{0.577 } & \textbf{0.371 } & 0.684  & 0.422  & \textbf{0.635 } & \textbf{0.411 } & 0.945  & 0.530  & \textbf{0.861 } & \textbf{0.524 } \\
\cmidrule{2-22}          & \textbf{$\uparrow$} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{10.25\%} & \textbf{5.55\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{18.28\%} & \textbf{7.57\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{9.77\%} & \textbf{3.70\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{8.61\%} & \textbf{4.80\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{11.19\%} & \textbf{1.65\%} \\
          & $\delta$ & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-2.879 \& -2.171}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-2.488 \& -2.201}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-2.254 \& -2.265}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-2.507 \& -2.304}}} & \multicolumn{4}{c}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-2.762 \& -2.238}}} \\
    \midrule
    \midrule
    \rotate{\textbf{ETTh1}} & \textbf{96 } & 0.411  & 0.432  & \textbf{0.382 } & \textbf{0.415 } & 0.495  & 0.480  & \textbf{0.491 } & \textbf{0.478 } & 0.375  & 0.414  & \textbf{0.370 } & \textbf{0.410 } & 0.440  & 0.444  & \textbf{0.430 } & \textbf{0.442 } & 0.948  & 0.774  & \textbf{0.684 } & \textbf{0.586 } \\
          & \textbf{192 } & 0.419  & 0.444  & \textbf{0.396 } & \textbf{0.422 } & 0.543  & 0.505  & \textbf{0.538 } & \textbf{0.503 } & 0.427  & 0.448  & \textbf{0.420 } & \textbf{0.443 } & 0.487  & 0.472  & \textbf{0.480 } & \textbf{0.470 } & 1.009  & 0.786  & \textbf{0.759 } & \textbf{0.624 } \\
          & \textbf{336 } & 0.439  & 0.459  & \textbf{0.418 } & \textbf{0.443 } & 0.581  & 0.521  & \textbf{0.574 } & \textbf{0.518 } & 0.458  & 0.465  & \textbf{0.454 } & \textbf{0.462 } & 0.471  & 0.475  & \textbf{0.467 } & \textbf{0.473 } & 1.035  & 0.783  & \textbf{0.776 } & \textbf{0.640 } \\
          & \textbf{720 } & 0.504  & 0.514  & \textbf{0.473 } & \textbf{0.503 } & 0.569  & 0.534  & \textbf{0.562 } & \textbf{0.530 } & 0.482  & 0.495  & \textbf{0.478 } & \textbf{0.492 } & 0.543  & 0.528  & \textbf{0.542 } & \textbf{0.527 } & 1.153  & 0.845  & \textbf{0.948 } & \textbf{0.726 } \\
\cmidrule{2-22}          & \textbf{$\uparrow$} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{5.94\%} & \textbf{3.53\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{1.08\%} & \textbf{0.56\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{1.10\%} & \textbf{0.74\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{1.08\%} & \textbf{0.35\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{23.60\%} & \textbf{19.18\%} \\
          & $\delta$ & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-3.111 \& -2.767}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 0,  .439,  .753}{\textbf{-3.207 \& -3.019}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 0,  .439,  .753}{\textbf{-3.52 \& -2.463}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 0,  .439,  .753}{\textbf{-3.572 \& -2.321}}} & \multicolumn{4}{c}{\textcolor[rgb]{ 0,  .439,  .753}{\textbf{-3.83 \& -1.883}}} \\
    \midrule
    \midrule
    \rotate{\textbf{ETTh2}} & \textbf{96 } & 0.641  & 0.555  & \textbf{0.527 } & \textbf{0.544 } & 0.346  & 0.401  & \textbf{0.344 } & \textbf{0.399 } & 0.341  & 0.385  & \textbf{0.339 } & \textbf{0.383 } & 0.363  & 0.405  & \textbf{0.362 } & \textbf{0.404 } & 2.992  & 1.362  & \textbf{0.948 } & \textbf{0.727 } \\
          & \textbf{192 } & 1.262  & 0.814  & \textbf{0.834 } & \textbf{0.725 } & 0.437  & 0.447  & \textbf{0.430 } & \textbf{0.443 } & 0.433  & 0.441  & \textbf{0.432 } & \textbf{0.440 } & 0.450  & 0.447  & \textbf{0.449 } & \textbf{0.446 } & 6.256  & 2.091  & \textbf{1.791 } & \textbf{1.056 } \\
          & \textbf{336 } & 1.486  & 0.896  & \textbf{1.048 } & \textbf{0.835 } & 0.478  & 0.479  & \textbf{0.467 } & \textbf{0.472 } & 0.503  & 0.494  & \textbf{0.501 } & \textbf{0.491 } & 0.470  & 0.474  & \textbf{0.468 } & \textbf{0.471 } & 5.265  & 1.954  & \textbf{1.845 } & \textbf{1.079 } \\
          & \textbf{720 } & 1.220  & 0.848  & \textbf{0.906 } & \textbf{0.758 } & 0.488  & 0.492  & \textbf{0.474 } & \textbf{0.482 } & 0.479  & 0.485  & \textbf{0.478 } & \textbf{0.484 } & 0.484  & 0.491  & \textbf{0.483 } & \textbf{0.489 } & 4.038  & 1.673  & \textbf{2.020 } & \textbf{1.104 } \\
\cmidrule{2-22}          & \textbf{$\uparrow$} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{28.05\%} & \textbf{8.06\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{1.93\%} & \textbf{1.31\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{0.42\%} & \textbf{0.40\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{0.25\%} & \textbf{0.35\%} & \textcolor[rgb]{ 1,  0,  0}{} & \textcolor[rgb]{ 1,  0,  0}{} & \textbf{64.40\%} & \textbf{44.00\%} \\
          & $\delta$ & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-2.451 \& -1.149}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-3.067 \& -1.079}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 0,  .439,  .753}{\textbf{-3.733 \& -1.943}}} & \multicolumn{4}{c|}{\textcolor[rgb]{ 0,  .439,  .753}{\textbf{-3.967 \& -1.921}}} & \multicolumn{4}{c}{\textcolor[rgb]{ 1,  0,  0}{\textbf{-3.021 \& -1.513}}} \\
    \midrule
    \bottomrule
    \end{tabular}%
    } % 注意加的位置在\begin{tabular}和\end{tabular}前后
    \begin{tablenotes}
      \small
      \item Results of \textit{ETTm1}, \textit{ETTm2} and \textit{Weather} datasets are included in Table \ref{tbl:Main_Results_Part2} of Appendix \ref{sec:app_full_benchmark_results}, due to space limit.
    \end{tablenotes}
  \label{tbl:Main_Results_Part1}%
\end{table*}%



==> table/tuning_strategies.tex <==
% Table generated by Excel2LaTeX from sheet 'adapt_whole_model'
\begin{table*}[htbp]
  \centering
  \caption{Extended table of Figure \ref{fig:extra-tuning}: Performance comparison between adaptation on prediction layer versus adaptation on entire model. "/" indicates original forecasts without \method{SOLID}. \method{SOLID-P} denotes method \method{SOLID} is solely employed on \underline{P}rediction layer, while \method{SOLID-E} denotes \method{SOLID} on the \underline{E}ntire model. And "pl96" or "pl192" means that the prediction length is 96 or 192 respectively.}
  \small
  % \resizebox{\linewidth}{!}{  % 此处！表示根据根据宽高比进行自适应缩放，并且一定要加在tabular两端，而不是table两端。
    \begin{tabular}{c|c|cc|cc|cc|cc|cc|cc}
    \toprule
    \multicolumn{2}{c|}{\textbf{Dataset}}       & \multicolumn{2}{c|}{\textbf{ETTh1+pl96}} & \multicolumn{2}{c|}{\textbf{ETTh1+pl192}} & \multicolumn{2}{c|}{\textbf{Traffic+pl96}} & \multicolumn{2}{c|}{\textbf{Traffic+pl192}} & \multicolumn{2}{c|}{\textbf{Illness+pl24}} & \multicolumn{2}{c}{\textbf{Illness+pl36}} \\
    \midrule
    % \midrule
    \multicolumn{2}{c|}{\textbf{Metric}} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} \\
    \midrule
    \midrule
    \textbf{Informer} & \textbf{/} & 0.948  & 0.774  & 1.009  & 0.786  & 0.731  & 0.406  & 0.739  & 0.414  & 5.096  & 1.533  & 5.078  & 1.535  \\
          & \textbf{+\method{SOLID-P}} & \textbf{0.684 } & \textbf{0.586 } & \textbf{0.759 } & \textbf{0.624 } & \textbf{0.628 } & \textbf{0.393 } & \textbf{0.653 } & \textbf{0.413 } & \textbf{2.874 } & \textbf{1.150 } & \textbf{3.299 } & \textbf{1.243 } \\
          & \textbf{+\method{SOLID-E}} & 0.817  & 0.656  & 0.859  & 0.667  & 0.692  & 0.403  & 0.703  & 0.417  & 2.991  & 1.208  & 3.476  & 1.272  \\
    \midrule
    \midrule
    \textbf{Autoformer} & \textbf{/} & 0.440  & 0.444  & 0.487  & 0.472  & 0.621  & 0.391  & 0.713  & 0.417  & 3.314  & 1.245  & 2.733  & 1.078  \\
          & \textbf{+\method{SOLID-P}} & \textbf{0.430 } & \textbf{0.442 } & \textbf{0.480 } & \textbf{0.470 } & \textbf{0.565 } & \textbf{0.376 } & \textbf{0.599 } & \textbf{0.379 } & \textbf{2.737 } & \textbf{1.118 } & \textbf{2.540 } & \textbf{1.015 } \\
          & \textbf{+\method{SOLID-E}} & 0.436  & 0.443  & 0.482  & \textbf{0.470 } & 0.597  & 0.385  & 0.605  & 0.403  & 2.891  & 1.150  & 2.655  & 1.068  \\
    \midrule
    \midrule
    \textbf{FEDformer} & \textbf{/} & 0.375  & 0.414  & 0.427  & 0.448  & 0.574  & 0.356  & 0.612  & 0.379  & 3.241  & 1.252  & 2.576  & 1.048  \\
          & \textbf{+\method{SOLID-P}} & \textbf{0.370 } & \textbf{0.410 } & \textbf{0.420 } & \textbf{0.443 } & \textbf{0.513 } & \textbf{0.344 } & \textbf{0.549 } & \textbf{0.361 } & \textbf{2.707 } & \textbf{1.123 } & \textbf{2.365 } & \textbf{0.990 } \\
          & \textbf{+\method{SOLID-E}} & 0.373  & 0.413  & 0.425  & 0.447  & 0.539  & 0.348  & 0.562  & 0.366  & 2.874  & 1.201  & 2.533  & 1.040  \\
    \midrule
    \midrule
    \textbf{ETSformer} & \textbf{/} & 0.495  & 0.480  & 0.543  & 0.505  & 0.599  & 0.386  & 0.611  & 0.391  & 2.397  & 0.993  & 2.504  & 0.970  \\
          & \textbf{+\method{SOLID-P}} & \textbf{0.491 } & \textbf{0.478 } & \textbf{0.538 } & \textbf{0.503 } & \textbf{0.487 } & \textbf{0.354 } & \textbf{0.492 } & \textbf{0.354 } & \textbf{2.262 } & \textbf{0.955 } & \textbf{2.301 } & \textbf{0.934 } \\
          & \textbf{+\method{SOLID-E}} & 0.492  & 0.479  & 0.541  & 0.504  & 0.517  & 0.368  & 0.523  & 0.374  & 2.353  & 0.986  & 2.339  & 0.965  \\
    \midrule
    \midrule
    \textbf{Crossformer} & \textbf{/} & 0.411  & 0.432  & 0.419  & 0.444  & 0.521  & 0.297  & 0.523  & 0.298  & 3.329  & 1.275  & 3.392  & 1.185  \\
          & \textbf{+\method{SOLID-P}} & \textbf{0.382 } & \textbf{0.415 } & \textbf{0.396 } & \textbf{0.422 } & \textbf{0.473 } & \textbf{0.267 } & \textbf{0.475 } & \textbf{0.270 } & \textbf{2.397 } & \textbf{1.052 } & 2.527  & 1.042  \\
          & \textbf{+\method{SOLID-E}} & 0.401  & 0.427  & 0.399  & 0.428  & 0.493  & 0.273  & 0.497  & 0.275  & 2.653  & 1.074  & \textbf{2.523 } & \textbf{1.017 } \\
    \midrule
    \bottomrule
    \end{tabular}%
    % } % 注意加的位置在\begin{tabular}和\end{tabular}前后
    \label{tbl:adapt_whole_model}
\end{table*}%


